GenCA: A Text-conditioned Generative Model for Realistic and Drivable Codec Avatars

Photo-realistic and controllable 3D avatars are crucial for various applications such as virtual and mixed reality (VR/MR), telepresence, gaming, and film production. Traditional methods for avatar creation often involve time-consuming scanning and reconstruction processes for each avatar, which limits their scalability. Furthermore, these methods do not offer the flexibility to sample new identities or modify existing ones. On the other hand, by learning a strong prior from data, generative models provide a promising alternative to traditional reconstruction methods, easing the time constraints for both data capture and processing. Additionally, generative methods enable downstream applications beyond reconstruction, such as editing and stylization. Nonetheless, the research on generative 3D avatars is still in its infancy, and therefore current methods still have limitations such as creating static avatars, lacking photo-realism, having incomplete facial details, or having limited drivability. To address this, we propose a text-conditioned generative model that can generate photo-realistic facial avatars of diverse identities, with more complete details like hair, eyes and mouth interior, and which can be driven through a powerful non-parametric latent expression space. Specifically, we integrate the generative and editing capabilities of latent diffusion models with a strong prior model for avatar expression driving. Our model can generate and control high-fidelity avatars, even those out-of-distribution. We also highlight its potential for downstream applications, including avatar editing and single-shot avatar reconstruction.

==> 6_figureonly.tex <==
% \clearpage
% \input{figures/ablation}
% \input{figures/monalisa_attributes}

% \input{figures/main_results}

% \begin{figure*}[h]
% 	\centering
%  	\begin{minipage}{0.48\linewidth}
% 		\centering
%   \vspace{-7mm}
% 	\includegraphics[width=9cm]
%  {figures/monalisa_attributes.png}
% \vspace{-0.5cm}
% \caption{Example of extracting attributes and generating text caption.}
%     \label{fig:data:anno}
% 	\end{minipage}
%         \hfill
% 	\begin{minipage}{0.48\linewidth}
% 	\centering
%  \vspace{-7mm}
% \includegraphics[width=9cm]{figures/ablation.pdf}
% \vspace{-0.5cm}
% \caption{Ablation study by disabling different parts of the proposed method. }
%     % \vspace{-10pt}
% \vspace{-0.35cm}
%     \label{fig:exp:ablation}
% 	\end{minipage}
% \end{figure*}


% \clearpage




% \clearpage


==> figures/ablation.tex <==
\begin{figure} [t!]
    \centering
    \includegraphics[trim = 5mm 5mm 0mm 5mm, width=0.45\textwidth]{figures/ablation.pdf}
    \caption{Ablation study by disabling different parts of the proposed method. }
    \label{fig:exp:ablation}
\end{figure}


==> figures/cmp_sota.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[trim = 0 0 0mm 0,  width=0.75\textwidth]{figures/cmp_sota.pdf}
    \vspace{-0.5cm}
    \caption{Qualitative comparison of \genca generation with three state-of-the-art methods. Compared to other methods, \genca produces more comprehensive and photorealistic avatars given the same text descriptions.}
    \label{fig:exp:cmp_sota}
\end{figure*}
% [ clip, width=0.5\textwidth]

==> figures/gca_teaser.tex <==
% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=0.9\textwidth]{figures/gca_teaser.png}
%     \caption{Teaser.\todo{placeholder}}
%     \label{fig:teaser}
% \end{figure*}

\begin{teaserfigure}
\centering
  \includegraphics[trim = 0 0 0mm 0, width=0.96\textwidth]
  % [left, bottom, right, top]
  {figures/teaser.pdf}
  \vspace{-0.4cm}
  \caption{\textbf{Generative Codec Avatars.} Given a sentence describing the attributes of a face, our method generates a Codec Avatar, which can be driven by realistic expressions (top). \genca has many downstream applications such as avatar reconstruction from a single in-the-wild image (bottom). Additionally, it allows for editing features, such as changing hair color to green (top) or removing facial hair (bottom).
  }
  \label{fig:teaser}
\end{teaserfigure}

==> figures/monalisa_attributes.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[trim = 0 0 0mm 16mm,  width=0.4\textwidth]{figures/monalisa_attributes.png}
    \caption{Example of extracting attributes and generating text caption.}
    % \vspace{-10pt}
    \label{fig:data:anno}
\end{figure}
% [ clip, width=0.5\textwidth]
% trim = left, bottom, right, top

==> tables/cmp_metrics_with_sota.tex <==
\begin{table*}
\centering
\captionsetup{justification=centering} % Centering the caption
\caption{Comparison with three state-of-the-art Methods. The three numbers for User Study denote: Semantic Alignment/Visual Appealing/Overall Preference}
\vspace{-3mm}
\begin{tabular}{lccccc}
\toprule
Method                    &    Venue    & CLIP Score & Aesthetic Score & HPS v2 & User Study \\
\midrule
Describe3D~\cite{describe3d}    & CVPR'23    & 17.71      & 4.581          & 0.1510 &        0.61\% / \underline{7.88\%} / 4.85\%    \\
DreamFace~\cite{dreamface}  &SIGGRAPH'23        & 17.70 & \underline{4.720} & 0.1605  & 2.42\% / 7.27\% / 6.06\%          \\
% Ours & 23.04 &  4.897& 0.1740\\
TADA~\cite{tada}      &3DV'24              & \textbf{17.83}      & 4.471          & \underline{0.1635} & \underline{32.73\%} / 1.21\% / \underline{6.06\%} \\
Ours                  &-              & \underline{17.82}      & \textbf{4.799}          & \textbf{0.1731} & \textbf{64.24\%} / \textbf{83.64\%} / \textbf{83.03\%} \\
\bottomrule
\end{tabular}
\vspace{-3mm}
\label{tab:sotacomparison}
\end{table*}

% 	                 clipscore	aes score	hps v2
% describe3d	   17.70898488	4.581161033	0.1510009766
% dreamface	        17.69747419	4.719701242	0.1605224609
% tada	         17.8291048	4.470887343	0.1634521484
% gca	          17.81973146	4.798755879	0.1730957031

==> tables/cmp_with_priors_in_concept.tex <==
\begin{table}
\captionsetup{justification=centering} % Centering the caption
\caption{Comparison between our proposed method (GenCA) and state-of-the-art methods~\cite{describe3d}, \cite{tada}, \cite{dreamface}}
\begin{tabular}{lcccc}
\toprule
                                    & Feed-Forward & High Res & Neural Render \\
\midrule
Describe3D        &   \ding{51}   &   \ding{55}   &   \ding{55}               \\
TADA                    &   \ding{55}   &   \ding{55}   &   \ding{55}               \\
DreamFace          &   \ding{55}   &   \ding{51}   &   \ding{55}               \\
GenCA (ours)                                &   \ding{51}   &   \ding{51}   &   \ding{51}               \\
\bottomrule
\end{tabular}
\label{tab:sotaconcept}
\end{table}
